Experimental results : Reinforcement Learning of POMDPs using Spectral Methods

We propose a new reinforcement learning algorithm for partially observable Markov decision processes (POMDP) based on spectral decomposition methods. While spectral methods have been previously employed for consistent learning of (passive) latent variable models such as hidden Markov models, POMDPs are more challenging since the learner interacts with the environment and possibly changes the future observations in the process. We devise a learning algorithm running through epochs, in each epoch we employ spectral techniques to learn the POMDP parameters from a trajectory generated by a fixed policy. At the end of the epoch, an optimization oracle returns the optimal memoryless planning policy which maximizes the expected reward based on the estimated POMDP model. We prove an order-optimal regret bound with respect to the optimal memoryless policy and efficient scaling with respect to the dimensionality of observation and action spaces.

==> 3pomdp_proof.tex <==
% !TEX root = master.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LEARNING POMDP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Lemma~\ref{lem:pomdp.parameters}}\label{s:proof.lem:pomdp.parameters}

The proof proceeds by construction. First notice that the elements of the second view can be written as
%
\begin{align*}
[V_2^{(l)}]_{s,i} &= [V_2^{(l)}]_{(n',m'),i}\\
&= \Prob(\vecy_2=\vec{e}_{n'}|x_2=i,a_2=l)\Prob(\vec{r}_2=\vec{e}_{m'}|x_2=i,a_2=l)\\
&= \Prob(\vecy_2=\vec{e}_{n'}|x_2=i,a_2=l) f_R(\vec{e}_{m'}|i,l),
\end{align*}
%
where we used the independence between observations and rewards. As a result, summing up over all the observations $n'$, we can recover the reward model as
%
\begin{align}
f_R(\vec{e}_{m'}|i,l) = \sum_{n'=1}^Y [V_2^{(l)}]_{(n',m'),i},
\end{align}
%
for any combination of states $i\in [X]$ and actions $l\in[A]$.
In order to compute the observation model, we have to further elaborate the definition of $V_2^{(l)}$ as
%
\begin{align*}
&[V_2^{(l)}]_{s,i} = [V_2^{(l)}]_{(n',m'),i}\\
&= \frac{\Prob(a_2=l|x_2=i,\vecy_2=\vec{e}_{n'}) \Prob(\vecy_2=\vec{e}_{n'}|x_2=i)}{ \Prob(a_2=l|x_2=i) } \cdot \Prob(\vec{r}_2=\vec{e}_{m'}|x_2=i,a_2=l) \\
&= \frac{f_\pi(l|\vec{e}_{n'}) f_O(\vec{e}_{n'}|i) f_R(\vec{e}_{m'}|i,l)}{\Prob(a_2=l|x_2=i)}.
\end{align*}
%
Since the policy $f_\pi$ is known, if we divide the previous term by $f_\pi(l|\vec{e}_{n'})$ and sum over observations and rewards, we obtain the denominator of the previous expression as
%
\begin{align*}%\label{eq:rho.term}
\sum_{m'=1}^R \sum_{n'=1}^Y \frac{[V_2^{(l)}]_{(n',m'),i}}{f_\pi(l|\vec{e}_{n'})} = \frac{1}{\Prob(a_2=l|x_2=i)}.
\end{align*}
%
Let $\rho(i,l) = 1/\Prob(a_2=l|x_2=i)$ as computed above, then the observation model is
%
\begin{align}
f^{(l)}_O(\vec{e}_{n'}|i) = \sum_{m'=1}^R \frac{[V_2^{(l)}]_{(n',m'),i}}{f_\pi(l|\vec{e}_{n'})\rho(i,l)}.
\end{align}
%
Repeating the procedure above for each $n'$ gives the full observation model $f_O^{(l)}$. We are left with the transition tensor, for which we need to resort to the third view $V_3^{(l)}$, that can be written as
%
\begin{align}\label{eq:v3.transition}
[V_3^{(l)}]_{s,i} &= [V_3^{(l)}]_{n'',i}\nonumber\\
&= \sum_{j=1}^X \Prob(\vecy_3=\vec{e}_{n''}|x_2=i,a_2=l, x_3=j)\cdot\Prob(x_3=j|x_2=i,a_2=l) \nonumber\\
&= \sum_{j=1}^X\Prob(\vecy_3=\vec{e}_{n''}|x_3=j)\Prob(x_3=j|x_2=i,a_2=l) \nonumber\\
&= \sum_{j=1}^X f_O(\vec{e}_n|j) f_T(j| i,l),
\end{align}
%
\noindent where we used the graphical model of the POMDP to introduce the dependency on $x_3$. Since the policy $f_\pi$ is known and the observation model is obtained from the second view with Eq.~\ref{eq:obs.recovery}, it is possible to recover the transition model. 
We recall that the observation matrix $O\in\Re^{Y\times X}$ is such that $[O]_{n,j} = f_O(\vec{e}_n|j)$, then we can restate Eq.~\ref{eq:v3.transition} as
%
\begin{align}\label{eq:transition.recovery}
O [T]_{i,:,l} = [V_3^{(l)}]_{:,i}
\end{align}
%
where $[T]_{i,:,l}$ is the second mode of the transition tensor $T\in\Re^{X\times X\times A}$. Since all the terms in $O$ are known, we finally obtain $[T]_{i,:,l} = O^\dagger [V_3^{(l)}]_{:,i}$, where $O^\dagger$ is the pseudo-inverse of $O$. Repeating for all states and actions gives the full transition model $f_T$.


==> Cextension.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LIMITED MEMORY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Extension to Bounded-Memory Policies}\label{app:bounded.memory}

\begin{figure}[h]
\tiny
\begin{center}
\begin{psfrags}
\psfrag{x1}[][1]{$x_0$}
\psfrag{x2}[][1]{$x_{1}$}
\psfrag{x3}[][1]{$x_{2}$}
\psfrag{x0}[][1]{$x_{-1}$}
\psfrag{y1}[][1]{$\vecy_0$}
\psfrag{y2}[][1]{$\vecy_{1}$}
\psfrag{y0}[][1]{$\vecy_{-1}$}
\psfrag{r1}[][1]{$r_0$}
\psfrag{r2}[][1]{$r_{1}$}
\psfrag{r0}[][1]{$r_{-1}$}
\psfrag{a1}[][1]{$a_{0}$}
\psfrag{a2}[][1]{$a_{1}$}
\psfrag{a0}[][1]{$a_{-1}$}
\includegraphics[width=0.45\textwidth,natwidth=810,natheight=642,trim={0 1.5cm 2cm 0.5cm},clip]{figs/I-6.eps}
\end{psfrags}
\end{center}
\caption{Bounded-Memory POMDP when \past=2.}
\label{fig:I-6}
\end{figure}


Throughout the paper we consider memory-less policies which only consider the current observation to decide which action to take. Nonetheless, our method, and notably the process of estimation of the POMDP parameters, can be easily extended to the case of bounded-memory policies. Let $\pi$ be a policy such that at time $t$ all the past $\past$ observations are considered to decide the action, that is $f_\pi(a|\vec{y}_t, \vec{y}_{t-1},\ldots,\vec{y}_{t-\past})$. In Fig.~\ref{fig:I-6} we illustrate the case for $\past=2$. In this case, we have to redefine the notion of views that we introduced in Sect.~\ref{s:learning.pomdp}. We define the first view $(\vecy_{-(\past-1)},a_{-(\past-1)},r_{-(\past-1)},\ldots,\vecy_{(-1)},a_{(-1)},r_{(-1)})$, the second view $(\vecy_0,r_0)$, and the third view $(\vecy_{(1)},r_{(1)},\ldots,\vecy_{(\past-1)},r_{(\past-1)})$. Given state $x_0$ and all actions $a_0,\ldots,a_{\past-1}$, it is easy to see that these views are independent and the multi-view model can be applied by extending the definitions of $V_{\nu}^{(l)}$ to this case. If the views satisfy the assumption of being full column rank, then all the results presented in Sect.~\ref{s:learning.pomdp} can be easily extended.




Usually, in the real systems, the agents do not make decision at each time step, even they do not apply their decision at each time step because usually making decision and applying that is expensive for agents. Lets take a look at the system that the agent chooses an action based on $p$ previous observation (including current observation) and then for $p-1$ time step, it just looks at the system and records the data, after that, based on this collected data, it choose new action. This model is simpler that the above mentioned model which we are not able to investigate it in this draft.  The simpler model is as follow. Let us consider the case of $p=2$, then
\begin{equation}
\begin{split}
&[\obs_1^{a_0=i}]_{l,f}=Pr(\vecy_{-1}=\vec{e}_j,r_{-1}=\vec{e}_b,a_{-1}=c|x_0=f)\\
&[\obs_2^{a_0=i}]_{l,f}=Pr(\vecy_0=\vec{e}_{j'},r_0=\vec{e}_{b'}|x_0=f,a_0=i)\\
&[\obs_3^{a_2=i}]_{l,f}=Pr(\vecy_1=\vec{e}_j,r_1=\vec{e}_b|x_0=f,a_0=i)
\end{split}
\end{equation}
The full rank condition is satisfied if either $\obs$ matrix or $R$ matrix is full column rank and transition matrix is full rank. Same idea as before, the agent do the learning part for each action and for each of them once it looks at third view as a third effect and once second view as a third view. By this it can learn $\obs$ and $\trans^{(a_0=i)}$ for all $i$. Addition to that, the agent need to find out the transition matrix when during passive time which is for example transition form $x_{-1}$ to $x_0$. To learn this part of model, the agent needs to estimate another set of $\obs$ matrices whose columns are conditioned on $x_1$, $i.e.$:
\begin{equation}
\begin{split}
&[\obs_1]_{l,f}=Pr(\vecy_{0}=\vec{e}_j,r_{0}=\vec{e}_b,a_{0}=c|x_1=f)\\
&[\obs_2]_{l,f}=Pr(\vecy_1=\vec{e}_{j'},r_1=\vec{e}_{b'}|x_1=f)\\
&[\obs_3]_{l,f}=Pr(\vecy_2=\vec{e}_j,r_2=\vec{e}_b,a_2=c|x_1=f)
\end{split}
\end{equation}
this set of $\obs$ gives us the transition matrix.




==> Concentration.tex <==
% !TEX root = master.tex

\section{Concentration Bound}\label{app:ConBound}

\begin{theorem}[Matrix Azuma]
Consider Hidden Markov Model with finite sequence of $n$ samples $S_i$ as observations given arbitrary initial states distribution and $c-Lipschitz$ matrix valued function $\Phi:S_{1}^{n}\rightarrow \mathbb{R}^{d_1\times d_2}$ in dimension $d_1$ by $d_2$, then
\begin{align*}
\left\|\Phi-\mathbb{E}[\Phi]\right\|_2\leq \frac{1}{1-\theta}\sqrt{8c^2n\log(\frac{(d_1+d_2)}{\delta})}
\end{align*}
with probability at least $1-\delta$. The $\mathbb{E}[\Phi]$ is given same initial distribution of samples.
\label{thm:MatrixAzuma}
\end{theorem}
\begin{proof}
The Thm.~ 7.1 \cite{tropp2012user} presents the upper confidence bound over the summation of matrix random variables. Consider a finite sequence of $d$ by $d'$ matrix $\Psi_i$, then for variance parameter $\sigma^2$ which is upper bound for $\sum_i\left[\Psi_i-\mathbb{E}_{i-1}[\Psi_i]\right],~~\forall i$
\begin{align*}
\left\|\sum_i\left[\Psi_i-\mathbb{E}_{i-1}[\Psi_i]\right]\right\|_2\leq \sqrt{8\sigma^2 \log(\frac{d+d'}{\delta})}
\end{align*}
with probability at least $1-\delta$.\\
For the function $\Phi$, lets define the martingale difference of function $\Phi$ as the input random variable with arbitrary initial distribution over states.
\begin{align*}
MD_i(\Phi;S_1^i)=\mathbb{E}[\Phi|S_1^i]-\mathbb{E}[\Phi|S_1^{i-1}]
\end{align*}
where $S_i^j$ is sub set of samples from $i'th$ position in sequence to $j'th$ one.
then the summation over these set of random variable gives $\mathbb{E}[\Phi|S_1^n]-\mathbb{E}[\Phi]$ which is  $\Phi(S_1^n)-\mathbb{E}[\Phi]$ and $\mathbb{E}[\Phi]$ is expectation with same initial state distribution . The remaining part is finding $\sigma$ which is upper bound for $\left\|\sum_iMD_i(\Phi;S_1^i)\right\|_2$ for all possible sequence. Lets define  $MD_i(\Phi)=\max_{S_1^i}MD_i(\Phi;S_1^i)$ and through \cite{kontorovich2008concentration} it is easy to show that $\left\|MD_i(\Phi)\right\|_2$ is $c-Lipchitz$ function and it is upper bounded by $cH_{i,n}$. In \cite{kontorovich2014uniform} it is shown that $H_{i,n}$ is upper bounded by $G\theta(n-i)$.
\end{proof}
For the case when $\Phi$ is symmetric matrix, $d_1+d_2$ can be reduced to just $d$ and constant $8$ can be reduced to $2$. \\
The result in Thm.~ \ref{thm:MatrixAzuma} can be extended to the situation when distribution of next state depends on current state and current observation and even more complicated models like memory-less policy POMDP.
\begin{theorem}[Concentration Bound]
Consider finite sequence of multiple views are drawn from memory less policy POMDP with common middle action and their corresponding covariance matrix $\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}$ for $\nu,\nu'\in\{1,2,3\}$ and $\nu\neq \nu'$. For simplicity, lets just consider one set of $\nu,\nu'$, one specific middle action, and $n$ samples are drawn. Define random variable $\Phi_i:=\frac{1}{N(l)}\left[\mathbb{E}\left[\sum_t\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\Big|S_1^{i}\right]-\mathbb{E}\left[\sum_t\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\Big|S_1^{i-1}\right]\right]$ with dimensions $d_\nu\times d_{\nu'}$ where $d_\nu$ and $d_{\nu'}$ for $\nu,\nu'\in \{1,2,3\}$ are the dimension along the $\nu$ and ${\nu}'$ views.
\begin{align*}
\left\|\sum_i\Phi_i\right\|_2=\left\|\frac{1}{N(l)}\sum_t\Big[\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\Big]-\frac{1}{N(l)}\mathbb{E}[\sum_t\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}]\right\|_2\leq \frac{G(\pi)}{1-\theta(\pi)}\sqrt{8\frac{\log\frac{(d_{\nu}+d_{\nu'})}{\delta}}{N(l)}}
\end{align*}
with probability at least $1-\delta$.\\
For tensor case, $\frac{1}{N(l)}\left[\mathbb{E}\left[\sum_t\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\otimes \vec{v}_{\nu'',t}^{(l)}\Big|S_1^{i}\right]-\mathbb{E}\left[\sum_t\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\otimes \vec{v}_{\nu'',t}^{(l)}\Big|S_1^{i-1}\right]\right]$ where $[\nu,\nu',\nu'']$ can be any permutation of set $\{1,2,3\}$.
\begin{align*}
\left\|\frac{1}{N(l)}\sum_t\Big[\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\otimes \vec{v}_{\nu'',t}^{(l)}\Big]-\frac{1}{N(l)}\mathbb{E}[\sum_t\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\otimes \vec{v}_{\nu'',t}^{(l)}]\right\|_2\leq\frac{G(\pi)}{1-\theta(\pi)} \sqrt{8\frac{\log\frac{(d_\nu d_{\nu'}+d_{\nu''})}{\delta}}{N(l)}}
\end{align*}
with probability at least $1-\delta$.
\label{thm:ConcentrationBound}
\end{theorem}
\begin{proof}
%Define random variable $S_t=\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}-\mathbb{E}_{t-1}[\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}]$


For simplicity lets just proof the first claim in Thm.~ \ref{thm:ConcentrationBound} and the proof for the second claim would be followed by same procedure. To proof the Thm.~\ref{thm:ConcentrationBound} it is needed to bring together the results from \cite{tropp2012user}, \cite{kontorovich2008concentration}, Thms.~ \ref{thm:GeneralConcentrationBound} , and \ref{thm:MatrixAzuma} and then modify them. The Thm.~ 7.1 in \cite{tropp2012user} presents following upper confidence bounds
\begin{align*}
\left\|\frac{1}{N(l)}\sum_t\Big[\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\Big]-\frac{1}{N(l)}\mathbb{E}[\sum_t\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}]\right\|_2\leq \sqrt{8(\widetilde{\sigma}_{Pairs}^{\nu,\nu'})^2\log\frac{(d_{\nu}+d_{\nu'})}{\delta}}
\end{align*}
with probability at least $1-\delta$. And
\begin{align*}
\left\|\frac{1}{N(l)}\sum_t\Big[\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\otimes \vec{v}_{\nu'',t}^{(l)}\Big]-\frac{1}{N(l)}\mathbb{E}[\sum_t\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\otimes \vec{v}_{\nu'',t}^{(l)}]\right\|_2\leq \sqrt{8(\widetilde{\sigma}_{Triples}^{\nu,\nu',\nu''})^2\log\frac{(d_\nu d_{\nu'}+d_{\nu''})}{\delta}}
\end{align*}
with probability at least $1-\delta$. It is needed to show that $(\widetilde{\sigma}_{Pairs}^{i,i'})^2\leq \frac{G(\pi)^2}{n(1-\theta(\pi))^2}$ and $(\widetilde{\sigma}_{Triples}^{i,i',i''})^2\leq \frac{G(\pi)^2}{n(1-\theta(\pi))^2}$.\\
\end{proof}

For the function $\Phi:S_1^n\rightarrow R^{d_1\times d_2}$, where $S_1^n$ is a collection of all possible $\{S_1,S_2, \ldots, S_n\}$ with length $n$. Its martingale difference is defined as follows
\begin{align*}
MD_i(\Phi;S_1^i)=\mathbb{E}[\Phi|S_1^i]-\mathbb{E}[\Phi|S_1^{i-1}]
\end{align*}
and then $MD_i(\Phi)=\max_{S_1^i}MD_i(\Phi;S_1^i)$.\\
The upper bound over $\widetilde{\sigma}_{Pairs}^{\nu,\nu'}$ is as follows
\begin{align*}
(\widetilde{\sigma}_{Pairs}^{\nu,\nu'})^2\leq \left\|\sum_{t=1}^nU_t^2\right\|_2
\end{align*}
Where $U_t$ is a fixed sequence of matrices which follows $MD_t\preceq U_t$ for all possible $MD_t$ and $\forall t$. This bound over Triple tensor can be derived after matricizing the martingale difference.
Next step is to upper bound the $\left\|\sum_tU_t^2\right\|_2$. \\
 Lets define new set of variables; given each action (middle action) $a_i=l$ there are the following set of variables; $\VV^{i|l}$ is collection of \\
$\vec{y}_{p(i,l)-1}, a_{p(i,l)-1}, r_{p(i,l)-1},\vec{y}_{p(i,l)}, r_{p(i,l)}, \vec{y}_{p(i,l)+1}$, \\
where $\VV^{i|l}$ is $i'th$ triple with middle action equal to $l$ and $p(i,l)$ is its corresponding position in the original sequence. Lets define variable $\HH^{i|l}$, which is consequence of four hidden states $x_{p(i,l)-1},x_{p(i,l)},x_{p(i,l)+1}, x_{p(i,l)+2}$. The variables $\VV^{j|l}_i$ and $\HH^{j|l}_i$, for $i\leq j$, are corresponding to set of consecutive $i\rightarrow j$ triple views and quadruple hidden states. Note that this is the time to define mixing coefficients.
\begin{align*}
\eta^{(l)}_{i,j}(\vv_1^{i-1|l},\varrho,\varrho'):=\left\|\mathbb{P}(\VV^{N(l)|l}_j|\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)-\mathbb{P}(\VV^{N(l)|l}_j|\VV^{i-1|l}_1=\vv_1^{i-1|l},\varrho',l)\right\|_{TV}
\end{align*}
where $TV$ is total variation distance between distributions and
\begin{align*}
\bar{\eta}^{(l)}_{i,j}:=\sup_{\vv_1^{i-1|l},\varrho,\varrho'}\eta^{(l)}_{ij}(\vv_1^{i-1|l},\varrho,\varrho')
\end{align*}
where $\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)$ and $\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho'.l)$ are nonzero for all possible input variables. Then for $\Delta_{N(l)}$ \\ \\
$(\Delta_{N(l)})_{i,j} =
\left\{
	\begin{array}{ll}
		1  & \mbox{if } i=j \\
		 \bar{\eta}^{(l)}_{i,j} & \mbox{if } i < j\\
		 0  & \mbox{ } otherwise.
	\end{array}
\right.$\\ \\
and $H_{n(l),i}=1+\bar{\eta}^{(l)}_{i,i+1}+\ldots+\bar{\eta}^{(l)}_{i,n}$






%which is upper bounded by $cH_{n,i}$. It means that $\sigma_{Triples}^2\leq \left\|\sum_i^nMD_i(\Phi))\right\|_2\leq nc^2\frac{1}{(1-\theta)^2}\leq \frac{1}{n(1-\theta)^2} $



\paragraph{Martingale Difference}.
To upper bound for $\widetilde{\sigma}_{Pairs}^{\nu,\nu'}$, it is enough to upper bound $\left\|\sum_{t=1}^nU_t^2\right\|_2$ or directly upper bound $\left\|\sum_{t=1}^nMD_t^2\right\|_2$ for all possible sequence of samples. The result in \cite{kontorovich2008concentration} shows that this is upper bounded by $\sum_{i=1}^{n(l)}\left\|MD_i(\Phi))\right\|^2_2$ and each $\left\|MD_i(\Phi))\right\|_2\leq cH_{n,i}$ when the $\left\|\Phi\right\|_2$ is $c-Lipschitz$. \\

In addition, it is obvious that for the class of moment functions with elements in $[0,1]$ the $c$ is upper bounded by $\frac{1}{N(l)}$ for the purpose of this paper. The remaining shows the upper bound over $H_{n,i}$ and then $\sum_{i=1}^{n(l)}H_{n,i}^2$.

\begin{lemma}
The function $H_{n,i}$ is upper bounded by $\frac{G(\pi)}{1-\theta(\pi)}$ and then $\sum_{i=1}^{n}(cH_{n,i})^2\leq nc^2\frac{G^2(\pi)}{(1-\theta(\pi))^2}\leq \frac{G^2(\pi)}{n(1-\theta(\pi))^2} $
\end{lemma}
\begin{proof}
As it mentioned, $H_{n(l),i}=1+\bar{\eta}^{(l)}_{i,i+1}+\ldots+\bar{\eta}^{(l)}_{i,n}$, and it is needed to find the upper bound over $1+\bar{\eta}^{(l)}_{i,i+1}+\ldots+\bar{\eta}^{(l)}_{i,n}$
\begin{align*}
&\eta^{(l)}_{ij}(\vv_1^{i-1|l},\varrho,\varrho')\\
&=\frac{1}{2}\sum_{\vv^{N(l)|l}_j}|\mathbb{P}(\VV^{N(l)|l}_j=\vv^{N(l)|l}_j|\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)-\mathbb{P}(\VV^{N(l)|l}_j=\vv^{N(l)|l}_j|\VV^{i-1|l}_1=\vv_1^{i-1|l},\varrho',l)|
\end{align*}
For the first part
\begin{align*}
&\mathbb{P}(\VV^{N(l)|l}_j=\vv^{N(l)|l}_j|\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)\\
&=\sum_{\hhh_1^{i|l},\hhh_j^{N(l)|l}}\mathbb{P}(\VV^{N(l)|l}_j=\vv^{N(l)|l}_j,\HH_1^{i|l}=\hhh_1^{i|l},\HH_j^{N(l)|l}=\hhh_j^{N(l)|l}|\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)
\end{align*}
Lets assume, for simplicity, that the hidden states on $\hhh^{i|l}$ do not have overlap with states on $\hhh^{i-1|l}$ and $\hhh^{i+1|l}$.
\begin{align*}
\mathbb{P}(\VV^{N(l)|l}_j&=\vv^{N(l)|l}_j|\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)=\\
&\sum_{\hhh_1^{i|l},\hhh_j^{N(l)|l}}\mathbb{P}(\VV^{N(l)|l}_j=\vv^{N(l)|l}_j,\VV^{i-1|l}_1=\vv_1^{i-1|l},\varrho,l|\HH_1^{i|l}=\hhh_1^{i|l},\HH_j^{N(l)|l}=\hhh_j^{N(l)|l})\\
&\mathbb{P}(\HH_1^{i|l}=\hhh_1^{i|l},\HH_j^{N(l)|l}=\hhh_j^{N(l)|l})\frac{1}{\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)}\\
&\hspace{-0cm}=\sum_{\hhh_1^{i|l},\hhh_j^{N(l)|l}}\mathbb{P}(\VV^{N(l)|l}_j=\vv^{N(l)|l}_j,l|\HH_j^{N(l)|l}=\hhh_j^{N(l)|l})\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l|\HH_1^{i|l}=\hhh_1^{i|l},\HH)\\
&\mathbb{P}(\HH_1^{i|l}=\hhh_1^{i|l},\HH_j^{N(l)|l}=\hhh_j^{N(l)|l})\frac{1}{\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)}
\end{align*}
with this representation
\begin{align*}
\eta^{(l)}_{ij}(\vv_1^{i-1|l},\varrho,\varrho')&=\frac{1}{2}\sum_{\vv_j^{N(l)|l}}|\sum_{\hhh_1^{i|l},\hhh_j^{N(l)|l}}\mathbb{P}(\VV^{N(l)|l}_j=\vv^{N(l)|l}_j|\HH_j^{N(l)|l}=\hhh_j^{N(l),l|l})\mathbb{P}(\HH_1^{i|l}=\hhh_1^{i|l},\HH_j^{N(l)|l}=\hhh_j^{N(l)|l})\\
&\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho',l|\HH_1^{i|l}=\hhh_1^{i|l})\big(\frac{\mathbb{P}(\varrho,l|\HH^{i|l}=\hhh^{i|l})}{\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)}-\frac{\mathbb{P}(\varrho',l|\HH^{i|l}=\hhh^{i|l})}{\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho',l)}\big)|
\end{align*}
\begin{align*}
\eta^{(l)}_{ij}(\vv_1^{i-1|l},\varrho,\varrho')&\leq \frac{1}{2}\sum_{\hhh^{j|l}}|\sum_{\hhh_1^{i|l}}\mathbb{P}(\VV^{N(l)|l}_j=\vv^{N(l)|l}_j,l|\HH_j^{N(l)|l}=\hhh_j^{N(l)|l})\mathbb{P}(\HH_1^{i|l}=\hhh_1^{i|l},\HH_j^{N(l)|l}=\hhh_j^{N(l)|l})\\
&\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho',l|\HH_1^{i|l}=\hhh_1^{i|l})\big(\frac{\mathbb{P}(\varrho,l|\HH^{i|l}=\hhh^{i|l})}{\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)}-\frac{\mathbb{P}(\varrho',l|\HH^{i|l}=\hhh^{i|l})}{\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho',l)}\big)|
\end{align*}
\begin{align*}
\eta^{(l)}_{ij}(\vv_1^{i-1|l},\varrho,\varrho')&\leq \frac{1}{2}\sum_{x^{p(j)-1|l}}|\sum_{\hhh_1^{i|l}}\mathbb{P}(\HH_1^{i|l}=\hhh_1^{i|l})\mathbb{P}(x^{p(j)-1|l}|x^{p(i,l)+2|l})\mathbb{P}(\VV^{i-1|l}_1=\vv_1^{i-1|l},l|\HH_1^{i|l}=\hhh_1^{i|l})q(\hhh^{i|l})|
\end{align*}
where
\begin{align*}
q(v,l):= \frac{\mathbb{P}(\varrho,l|\HH^{i|l}=v)}{\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)}-\frac{\mathbb{P}(\varrho',l|\HH^{i|l}=v)}{\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho',l)}
\end{align*}
then
\begin{align*}
\eta^{(l)}_{ij}(\vv_1^{i-1|l},\varrho,\varrho')&\leq \frac{1}{2}\sum_{x^{p(j)-1|l}}|\sum_{\hhh^{i|l}}\mathbb{P}(x^{p(j)-1|l}|x^{p(i,l)+2|l})h(\hhh^{i|l},l)|\\
&\leq \frac{1}{2}\sum_{x^{p(j)-1|l}}|\sum_{x^{p(i,l)+1|l}}\mathbb{P}(x^{p(j)-1|l}|x^{p(i,l)+2|l})\sum_{x^{p(i,l)+1|l},x^{p(i,l)|l},x^{p(i,l)-1|l}}h(\hhh^{i|l},l)|\\
&\leq \frac{1}{2}\sum_{x^{p(j)-1|l}}|\sum_{x^{p(i,l)+2|l}}\mathbb{P}(x^{p(j)-1|l}|x^{p(i,l)+2|l})\bar{h}(x^{p(i,l)+2|l},l)|
\end{align*}
where
\begin{align*}
h(v,l):=\sum_{\hhh_1^{i-1|l}}\mathbb{P}(\HH_1^{i|l}=\hhh_1^{i|l})\mathbb{P}(\VV^{i-1|l}_1=\vv_1^{i-1|l},l|\HH_1^{i|l}=\hhh_1^{i|l})q({v},l)
\end{align*}
%
%
\begin{align*}
\bar{h}(x^{p(i,l)+2|l},l):=\sum_{x^{p(i,l)+1|l},x^{p(i,l)|l},x^{p(i,l)-1|l}}h(\hhh^{i|l},l)
\end{align*}
as a consequence
\begin{align*}
\eta^{(l)}_{ij}(\vv_1^{i-1|l},\varrho,\varrho')\leq \left\|\frac{1}{2}\bar{h}^\top P^{i,j}\right\|_1
\end{align*}
where $P^{i,j}=\mathbb{P}(x^{p(j)-1|l}|x^{p(i,l)+2|l})$. Through Lemma A.2 in \cite{kontorovich2008concentration} and \cite{kontorovich2014uniform}, when $\sum_x{\bar{h}(x,l)}=0$ and $\frac{1}{2}\left\|\bar{h}\right\|_1\leq 1$, it is clear that $\eta^{(l)}_{ij}(\vv_1^{i-1|l},\varrho,\varrho')$, and also $\bar{\eta}^{(l)}_{ij}$ can be bounded by  $\frac{1}{2}\left\|\bar{h}^\top\right\|_1 G(\pi)\theta(\pi)^{p(j,l)-p(i,l)-4}$. To verify $\sum_x{\bar{h}}=0$ and $\frac{1}{2}\left\|\bar{h}\right\|_1\leq 1$
\begin{align*}
\sum_{x^{p(i,l)+2|l}}&\bar{h}(x^{p(i,l)+2|l},l)=\sum_{x^{p(i,l)+2|l}}\sum_{x^{p(i,l)+1|l},x^{p(i,l)|l},x^{p(i,l)-1|l}}h(\hhh^{i|l},l)=\sum_{\hhh^{i|l}}h(\hhh^{i|l},l)\\
&=\sum_{\hhh_1^{i|l}}\mathbb{P}(\HH_1^{i|l}=\hhh_1^{i|l})\mathbb{P}(\VV^{i-1|l}_1=\vv_1^{i-1|l},l|\HH_1^{i|l}=\hhh_1^{i|l})q({\hhh^{i|l}},l)\\
&=\sum_{\hhh_1^{i|l}}\mathbb{P}(\HH_1^{i|l}=\hhh_1^{i|l})\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},l|\HH_1^{i|l}=\hhh_1^{i|l}) \Bigg(\frac{\mathbb{P}(\varrho,l|\HH^{i|l}={\hhh^{i|l}})}{\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)}-\frac{\mathbb{P}(\varrho',l|\HH^{i|l}={\hhh^{i|l}})}{\mathbb{P}(\VV^{i-1|l}_1=\vv_1^{i-1|l},\varrho',l)}\Bigg)
\end{align*}
For the first part of parenthesis
\begin{align*}
\sum_{\hhh_1^{i|l}}\mathbb{P}(\HH_1^{i|l}=\hhh_1^{i|l})\mathbb{P}(\VV^{i-1|l}_1=\vv_1^{i-1|l},l|\HH_1^{i|l}=\hhh_1^{i|l}) \Bigg(\frac{\mathbb{P}(\varrho,l|\HH^{i|l}={\hhh^{i|l}})}{\mathbb{P}(\VV^{i|l}_1=\vv_1^{i-1|l},\varrho,l)}\Bigg)=1
\end{align*}
and same for the second one. This shows the conditions for the Lemma A.2 in \cite{kontorovich2008concentration}, $\sum_x{\bar{h}(x,l)}=0$ and $\frac{1}{2}\left\|\bar{h}\right\|_1\leq 1$, are met. \\
The presented proof is for the case of non-overlapped with states of $\HH^{i|l}$, for the other cases, the overlapped situation, the proof is pretty much similar to the non-overlapped case.
%The remaining part is bounding the parameter $\theta$ based on model parameters.
%
%\begin{align*}
%\theta=\sup_{x,x'}\left\|\ f_{T,\pi}(\cdot|x) -f_{T,\pi}(\cdot|x'&) \right\|_{TV}=\sup_{x,x'}\left\|T(x,I,\Pi Ox) -T(x',I,\Pi Ox')\right\|_{TV}\\
%&\leq  \sup_{i,j,i',j'\in [X]}\left\|T(\vec{e}_i,I,\vec{e_j}) -T(\vec{e}_{i'},I,\vec{e_{j'}})\right\|_{TV}\leq 1
%\end{align*}
%where $\Pi$ is $A\times Y$ policy matrix and $x$ and $x'$ are basis vectors.
 Now, it is the time to upper bound $\left\|\Delta_{N(l)}\right\|_\infty$.
\begin{align*}
H_{n,i}=1+\sum_{j=i}^{N(l)}\bar{\eta}^{(l)}_{ij}\leq 1+\max_i\sum_{j>i}\bar{\eta}^{(l)}_{ij}&\leq G(\pi)\sum_{i=0}^{n(l)}\theta(\pi)^{p(i,l)} \leq G(\pi)\sum_{i=0}^{n(l)}\theta(\pi)^{i}\\
&= G(\pi)\frac{1-\theta(\pi)^{n(l)}}{1-\theta(\pi)}\leq\frac{G(\pi)}{1-\theta(\pi)}
\end{align*}
\end{proof}
Define $\mathbb{E}_{stat}$ as the expectation with initial distribution equals to stationary distribution. Generally, in tensor decomposition, we are interested in
\begin{align*}
&\left\|\frac{1}{N(l)}\sum_t\Big[\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',i}^{(l)}\Big]-\frac{1}{N(l)}\mathbb{E}_{stat}[\sum_i\vec{v}_{\nu,t}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}]\right\|_2\\
&\left\|\frac{1}{N(l)}\sum_t\Big[\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',i}^{(l)}\otimes \vec{v}_{\nu'',i}^{(l)}\Big]-\frac{1}{N(l)}\mathbb{E}_{stat}[\sum_i\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',i}^{(l)}\otimes \vec{v}_{\nu'',i}^{(l)}]\right\|_2
\end{align*}
instead of
\begin{align*}
&\left\|\frac{1}{N(l)}\sum_t\Big[\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',i}^{(l)}\Big]-\frac{1}{N(l)}\mathbb{E}[\sum_i\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',i}^{(l)}]\right\|_2\\
&\left\|\frac{1}{N(l)}\sum_t\Big[\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',i}^{(l)}\otimes \vec{v}_{\nu'',i}^{(l)}\Big]-\frac{1}{N(l)}\mathbb{E}[\sum_i\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',t}^{(l)}\otimes \vec{v}_{\nu'',i}^{(l)}]\right\|_2
\end{align*}
which are derived through Thm.~ \ref{thm:ConcentrationBound}. To come up with the upper confidence bound over the above mentioned interesting deviation, it is needed to derive the upper bound for deviation over expectation with arbitrary initial state distribution and expectation with stationary distribution over initial states, for simplicity, lets just derive the bound for second order moment.
\begin{align*}
\left\|\frac{1}{N(l)}\mathbb{E}_{n}[\sum_i\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',i}^{(l)}]-\frac{1}{N(l)}\mathbb{E}_{stat}[\sum_i\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',i}^{(l)}]\right\|_2
\end{align*}
As the bound $\epsilon_i$ over deviation from stationary distribution of Markov chain follows $\epsilon=G(\pi)\theta(\pi)^{-i}$. It results in
\begin{align*}
\left\|\frac{1}{N(l)}\mathbb{E}[\sum_i\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',i}^{(l)}]-\frac{1}{N(l)}\mathbb{E}_{stat}[\sum_i\vec{v}_{\nu,i}^{(l)}\otimes \vec{v}_{\nu',i}^{(l)}]\right\|_2\leq 2\frac{G(\pi)}{N(l)(1-\theta(\pi))}
\end{align*}
which is negligible compared to $\widetilde{\mathcal{O}}(\frac{1}{\sqrt{n}})$ 
\begin{corollary}
These result hold for pure HMM model. For tensor case, where $[\nu,\nu',\nu'']$ is any permutation of set $\{1,2,3\}$.
\begin{align*}
\left\|\frac{1}{N(l)}\sum_t\Big[\vec{v}_{\nu,t}\otimes \vec{v}_{\nu',t}\Big]-\frac{1}{N}\mathbb{E}[\sum_t\vec{v}_{\nu,t}\otimes \vec{v}_{\nu',t}]\right\|_2\leq \frac{G}{1-\theta}\sqrt{8\frac{\log\frac{(d_{\nu}+d_{\nu'})}{\delta}}{N(l)}}
\end{align*}
with probability at least $1-\delta$ and\\

\begin{align*}
\left\|\frac{1}{N}\sum_t\Big[\vec{v}_{\nu,t}\otimes \vec{v}_{\nu',t}\otimes \vec{v}_{\nu'',t}\Big]-\frac{1}{N}\mathbb{E}[\sum_t\vec{v}_{\nu,t}\otimes \vec{v}_{\nu',t}\otimes \vec{v}_{\nu'',t}]\right\|_2\leq\frac{G}{1-\theta} \sqrt{8\frac{\log\frac{(d_\nu d_{\nu'}+d_{\nu''})}{\delta}}{N}}
\end{align*}
with probability at least $1-\delta$. The deviation bound is as follows
\begin{align*}
\left\|\frac{1}{N}\mathbb{E}[\sum_i\vec{v}_{\nu,i}\otimes \vec{v}_{\nu',i}]-\frac{1}{N}\mathbb{E}_{stat}[\sum_i\vec{v}_{\nu,i}\otimes \vec{v}_{\nu',i}]\right\|_2\leq 2\frac{G}{N(1-\theta)}
\end{align*}
\end{corollary}
\begin{proof}
Through \cite{kontorovich2008concentration} and \cite{kontorovich2014uniform} it is shown that for the HMM models, the value of $H_{n,i}$ is bounded by $\frac{G}{1-\theta}$ and then it means that the corresponding martingale difference is bounded by $\frac{cG}{1-\theta}$. In the consequence, the $\sigma^2_{HMM,\Phi}$ is bounded by $\frac{G^2}{n(1-\theta)^2}$.
\end{proof}

==> MainTheorem.tex <==
\section{Concentration Bound}\label{app:HMMConst}
\noindent\paragraph{Concentration of functions of a HMM}  We now provide concentration bounds for any matrix valued function $\phi(\cdot)$ over samples drawn from a HMM. This extends the result on scalar functions by~\citet{kontorovich2014uniform}.

For any ergodic Markov chain, lets consider $\omega$ as its stationary distribution and $f_{1\rightarrow t}(x_t|x_1)$ as a distribution over states at time $t$ given initial state $x_1$. Lets define inverse mixing time $\rho_{mix}(t)$ as follows
\begin{align*}
\rho_{mix}(t)=\sup_{x_1}\left\|f_{1\rightarrow t}(\cdot|x_1)-\omega\right\|_{TV}
\end{align*}
~\citet{kontorovich2014uniform} show  that this measure can be bounded by%\aacomment{replace with Roi's paper as ref}
\begin{align*}
\rho_{mix}(t)\leq G\theta^{t-1},
\end{align*}
where $1\leq G<\infty$ is $geometric$ $ergodicity$ and $0\leq \theta<1$ is contraction coefficient of Markov chain.

As before, let  $\bfy^n:=[\vec{y}_1, \ldots, \vec{y}_n]\in \calY^n$ denote the sequence of observations from HMM and let $x^n :=[x_1, \ldots, x_n]\in \calX^n$ denote the sequence of hidden states. We now consider matrix valued function $\Phi:\calY^{n}\rightarrow \mathbb{R}^{d_1\times d_2}$. It is said to be   $c$-Lipschitz  with respect to  spectral norm when
\begin{align*}
\sup_{\bfy^n, {\bfy'}^n \in \calY^n}\frac{\left\|\Phi(\bfy^n)-\Phi({\bfy'}^n)\right\|_2}{\|\bfy^n-{\bfy'}^n\|_H}\leq c
\end{align*}
where $\|\cdot\|_H$ is norm with respect to Hamming metric,   and $\bfy^n, {\bfy'}^n$ are any two sequences of  sample observations.
\begin{theorem}[HMM Concentration Bound]
Consider Hidden Markov Model with finite sequence of $n$ samples $\vec{y}_i$ as observations from finite observation set $\bfy^n$ and arbitrary initial state distribution. For any $c$-Lipschitz matrix valued function $\Phi(\cdot)$, we have
\begin{align*}
\left\|\Phi(\bfy^n)-\mathbb{E}[\Phi(\bfy^n)]\right\|_2\leq G\frac{1+\frac{1}{\sqrt{2}cn^{\frac{3}{2}}}}{1-\theta}\sqrt{8c^2n\log(\frac{(d_1+d_2)}{\delta})}
\end{align*}
with probability at least $1-\delta$, where G is  $geometric$ $ergodicity$ constant of corresponding Markov chain, and the $\mathbb{E}[\Phi(\bfy^n)]$ is expectation over samples of HMM when the initial distribution corresponds to the stationary distribution.
\label{thm:GeneralConcentrationBound}
\end{theorem}
\begin{proof}
In the Appendix. \ref{app:Proof_main}
\end{proof}
%Later, we extend this result  to the more complicated model of memory-less policy POMDP in order to derive our regret bounds. 
\begin{theorem}[POMDP Concentration Bound]
Consider Partially Observable Markov Decision Process with finite sequence of $n(l)$ samples $\vec{y}_i^{(l)}$ for all $i\in\lbrace1,2,\ldots,n(l)\rbrace~\forall l\in[A]$ as observations from finite observation sets $\bfy^{n(l)}$ and arbitrary initial state distribution. For any $c$-Lipschitz matrix valued function $\Phi^l(\cdot)$ function, we have
\begin{align*}
\left\|\Phi^l(\bfy^{n(l)})-\mathbb{E}[\Phi^l(\bfy^{n(l)})]\right\|_2\leq G\frac{1+\frac{1}{\sqrt{2}cn^{\frac{3}{2}}}}{1-\theta}\sqrt{8c^2n\log(\frac{(d_1+d_2)}{\delta})}
\end{align*}
with probability at least $1-\delta$, where G is  $geometric$ $ergodicity$ constant of corresponding Markov chain, and the $\mathbb{E}[\Phi(\bfy^{n(l)})]$ is expectation over samples of POMDP with middle action $l$ when the initial distribution corresponds to the stationary distribution.
\label{thm:GeneralConcentrationBoundPOMDP}
\end{theorem}
\begin{proof}
In the Appendix. \ref{app:Proof_main}
\end{proof}


==> macros.tex <==

%\mbox - function definitions
\def\tl{\tilde}\renewcommand\t{{\scriptscriptstyle\top}}

\newcommand\Dir{\operatorname{Dir}}
\newcommand\inner[1]{\ensuremath{\langle #1 \rangle}}
%\newcommand{\aacomment}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AA:} \textsf{#1} \#\#\#}}}
\newcommand{\mjcomment}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# MJ:} \textsf{#1} \#\#\#}}}
\newcommand{\hscomment}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# HS:} \textsf{#1} \#\#\#}}}
\def\indicator{{1{\hskip -2.5 pt}\hbox{I}}}
\DeclareMathOperator{\polylog}{polylog}
\newcommand\cov{\operatorname{Cov}}
 %\DeclareMathOperator{\short}{short}
\DeclareMathOperator{\sym}{Sym}
  \DeclareMathOperator{\tw}{tw}
  \DeclareMathOperator{\local}{local}
  \DeclareMathOperator{\range}{range}
   \DeclareMathOperator{\Path}{Path}
 \DeclareMathOperator{\Sg}{Sg}
 \DeclareMathOperator{\spt}{SP}
 \DeclareMathOperator{\avg}{avg}
  \DeclareMathOperator{\nbd}{\mathcal{N}}
 \DeclareMathOperator{\parent}{Pa}
 \DeclareMathOperator{\Cq}{Cq}
 \DeclareMathOperator{\TW}{TW}
 

 \DeclareMathOperator{\approxML}{ApproxML}
 \DeclareMathOperator{\Bethe}{Bethe}
 \DeclareMathOperator{\TRW}{TRW}
 \DeclareMathOperator{\conv}{Conv}
 \DeclareMathOperator{\lbp}{LBP}
 \DeclareMathOperator{\Corr}{Corr}
 \DeclareMathOperator{\hCorr}{\widehat{Corr}}
 \DeclareMathOperator{\hSc}{\widehat{\mathcal{S}}}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\mst}{MST}
\DeclareMathOperator{\supp}{supp}
 \DeclareMathOperator{\dtv}{d_{TV}}
 \DeclareMathOperator{\hdtv}{\hd_{TV}}
 \DeclareMathOperator*{\argmin}{arg\,min}
 \DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\essinf}{ess\,inf}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\rank}{Rank}
\DeclareMathOperator{\Krank}{Rank_K}
\DeclareMathOperator{\Det}{Det}
\DeclareMathOperator{\poiss}{Poiss}
\DeclareMathOperator{\unif}{Unif} \DeclareMathOperator{\Deg}{Deg}
\def\simiid{{\overset{i.i.d.}{\sim}}}
\def\lcv{{\,\,\underset{cv}{\leq}\,\,}}
\def\gcv{{\,\,\underset{cv}{\geq}\,\,}}
\def\lcx{{\,\,\underset{cx}{\leq}\,\,}}
\def\gcx{{\,\,\underset{cx}{\geq}\,\,}}
\def\leqst{{\,\,\overset{st}{\leq}\,\,}}
\def\geqst{{\,\,\overset{st}{\geq}\,\,}}
\def\eqdist{{\,\,\overset{d}{=}\,\,}}
\def\geqrh{{\,\,\overset{rh}{\geq}\,\,}}
\def\geqlr{{\,\,\overset{lr}{\geq}\,\,}}
\def\eqlr{{\,\,\overset{lr}{=}\,\,}}
\def\comment{{\mbox{\bf Comment\_Anima: }}}
\def\tha{{\mbox{\tiny th}}}

\DeclareMathOperator{\Aug}{Aug}
\DeclareMathOperator{\watts}{Watts}
\DeclareMathOperator{\girth}{Girth}
\DeclareMathOperator{\PL}{PL}
\DeclareMathOperator{\LP}{LP}
\DeclareMathOperator{\ER}{ER}
\DeclareMathOperator{\reg}{Reg}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\hSigma}{\widehat{\Sigma}}
%\DeclareMathOperator{\hrho}{\widehat{\rho}}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Poiss}{Poiss}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\Diam}{Diam}
\def\erf{\mbox{erf}}
\def\erfc{\mbox{erfc}}
\def\qfunc{\mbox{Q}}
%\def\myexp{\mbox{e}}
\def\snr{\mbox{{SNR}}}
\def\signum{\mbox{sgn}}
\def\Card{\mbox{Card}}
\DeclareMathOperator*{\plim}{plim}
\def\convd{\overset{d}\rightarrow}
\def\convp{\overset{p}\rightarrow}
\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\def\pl{{\parallel}}
%\DeclarePairedDelimiter\norm{\lVert}{\rVert}
%\DeclarePairedDelimiter\nuclearnorm{\lVert}{\rVert_*}
%\DeclarePairedDelimiter\onenorm{\lVert}{\rVert_1}
%\def\rinfnorm{\rVert_{\infty}}
%\DeclarePairedDelimiter\infnorm{\lVert}{\rinfnorm}
%\def\lnorm{{\lvert\!\lvert\!\lvert}}
%\def\rnorm{{\rvert\!\rvert\!\rvert}}
%\DeclarePairedDelimiter\gennorm{\lnorm}{\rnorm}
% \DeclarePairedDelimiter\abs{\lvert}{\rvert}
% \DeclarePairedDelimiter\geninfnorm{\lnorm}{\rnorm_{\infty}}
% \DeclarePairedDelimiter\genonenorm{\lnorm}{\rnorm_{1}}
\DeclareMathOperator{\atanh}{atanh}
 \DeclareMathOperator{\sech}{sech}
 \def\0{{\bf 0}}

\DeclareMathOperator{\lea}{\overset{(a)}{\leq}}
\DeclareMathOperator{\leb}{\overset{(b)}{\leq}}
\DeclareMathOperator{\lec}{\overset{(c)}{\leq}}
\DeclareMathOperator{\led}{\overset{(d)}{\leq}}
\DeclareMathOperator{\lee}{\overset{(e)}{\leq}}

\DeclareMathOperator{\eqa}{\overset{(a)}{=}}
\DeclareMathOperator{\eqb}{\overset{(b)}{=}}
\DeclareMathOperator{\eqc}{\overset{(c)}{=}}
\DeclareMathOperator{\eqd}{\overset{(d)}{=}}
\DeclareMathOperator{\eqe}{\overset{(e)}{=}}

\DeclareMathOperator{\gea}{\overset{(a)}{\geq}}
\DeclareMathOperator{\geb}{\overset{(b)}{\geq}}
\DeclareMathOperator{\gec}{\overset{(c)}{\geq}}
\DeclareMathOperator{\ged}{\overset{(d)}{\geq}}
\DeclareMathOperator{\gee}{\overset{(e)}{\geq}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% \algrenewcommand{\algorithmiccomment}[1]{// #1}
% \algrenewcommand{\algorithmicrequire}{\textbf{Input:}}
% \algrenewcommand{\algorithmicforall}{\textbf{for each}}


%text abbreviations
%\def\etal{{et al. \/}}
\def\viz{{viz.,\ \/}}
\def\ie{{i.e.,\ \/}}
\def\eg{{e.g.,\ \/}}
\def\etc{{etc.  }}
\def\ifff{{iff  }}
\def\as{{a.s.  }}
\def\st{{s.t.  }}
\def\wpone{{w.p.}\,1\,\,}
\def\wpp{{w.p.p.}\,\,}
\def\for{\,\,\mbox{for}\quad}
\def\ifmbox{\,\,\mbox{if}\quad}
\def\nn{\nonumber}
%\def\qed{\hfill$\Box$}
\def\ni{\noindent}

\def\qed{\hfill\hbox{${\vcenter{\vbox{
    \hrule height 0.4pt\hbox{\vrule width 0.4pt height 6pt
    \kern5pt\vrule width 0.4pt}\hrule height 0.4pt}}}$}}
\def\complx{\mathbb{C}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%ldp : use ldp.tex file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Detection on Graphs



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%colors
\def\tcr{\textcolor{red}}
\def\tcb{\textcolor{blue}}
\def\tcg{\textcolor{green}}
\def\tcw{\textcolor{white}}
\def\tcm{\textcolor{magenta}}
\def\tccyan{\textcolor{cyan}}
\def\tcv{\textcolor{violet}}
\definecolor{myred}{rgb}{0.3,0.0,0.7}
\definecolor{dkg}{rgb}{0.1,0.7,0.2}
\definecolor{dkb}{rgb}{0.0,0.2,0.8}

\def\tcdkb{\textcolor{dkb}}
\def\tcdkg{\textcolor{dkg}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\mathscr

\newcommand{\Amsc}{\mathscr{A}}
\newcommand{\Cmsc}{\mathscr{C}}
\newcommand{\Dmsc}{\mathscr{D}}
\newcommand{\Emsc}{\mathscr{E}}
\newcommand{\Fmsc}{\mathscr{F}}
\newcommand{\Gmsc}{\mathscr{G}}
\newcommand{\Hmsc}{\mathscr{H}}
\newcommand{\Kmsc}{\mathscr{K}}
\newcommand{\Nmsc}{\mathscr{N}}
\newcommand{\Pmsc}{\mathscr{P}}
\newcommand{\Qmsc}{\mathscr{Q}}
\newcommand{\Rmsc}{\mathscr{R}}
\newcommand{\Smsc}{\mathscr{S}}
\newcommand{\Tmsc}{\mathscr{T}}
\newcommand{\Umsc}{\mathscr{U}}
\newcommand{\Xmsc}{\mathscr{X}}
\newcommand{\Ymsc}{\mathscr{Y}}



%%%%%%%%%%%%%%%%%%%%%%hat
 \def\ha{\hat{a}}
 \def\hb{\hat{b}}
 \def\hc{\hat{c}}
\def\hd{\widehat{d}}
 \def\he{\widehat{e}}
 \def\hf{\hat{f}}
 \def\hg{\widehat{g}}
 \def\hh{\widehat{h}}
 \def\hi{\widehat{i}}
 \def\hj{\widehat{j}}
 \def\hk{\widehat{k}}
 \def\hl{\widehat{l}}
 \def\hm{\widehat{m}}
 \def\hn{\widehat{n}}
 \def\ho{\widehat{o}}
 \def\hp{\widehat{p}}
 \def\hq{\widehat{q}}
 \def\hr{\widehat{r}}
 \def\hs{\widehat{s}}
 \def\hatt{\widehat{t}}
 \def\hu{\hat{u}}
 \def\hv{\widehat{v}}
 \def\hw{\hat{w}}
 \def\hx{\hat{x}}
 \def\hy{\hat{y}}
 \def\hz{\widehat{z}}
% %bold caps
 \def\hA{\hat{A}}
 \def\hB{\hat{B}}
 \def\hC{\hat{C}}
 \def\hD{\widehat{D}}
 \def\hE{\widehat{E}}
 \def\hF{\widehat{F}}
 \def\hG{\widehat{G}}
 \def\hH{\widehat{H}}
 \def\hI{\widehat{I}}
 \def\hJ{\widehat{J}}
 \def\hK{\widehat{K}}
 \def\hL{\widehat{L}}
 \def\hM{\widehat{M}}
\def\hN{\widehat{N}}
 \def\hO{\widehat{O}}
 \def\hP{\widehat{P}}
 \def\hQ{\widehat{Q}}
 \def\hR{\widehat{R}}
 \def\hS{\widehat{S}}
\def\hT{\widehat{T}}
 \def\hU{\widehat{U}}
 \def\hV{\widehat{V}}
\def\hW{\widehat{W}}
 \def\hX{\hat{X}}
 \def\hY{\widehat{Y}}
 \def\hZ{\widehat{Z}}

 \def\hlambda{\widehat{\lambda}}
\def\hpi{\widehat{\pi}}
\def\hnu{\widehat{\nu}}
\def\hbd{\widehat{\mathbf{d}}}


\def\bLambda{\mathbf{\Lambda}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%bold alphabets
\def\bfzero{{\mathbf{0}}}
\def\bfone{{\mathbf{1}}}
\def\bfa{{\mathbf a}}
\def\bfb{{\mathbf b}}
\def\bfc{{\mathbf c}}
\def\bfd{{\mathbf d}}
\def\bfe{{\mathbf e}}
\def\bff{{\mathbf f}}
\def\bfg{{\mathbf g}}
\def\bfh{{\mathbf h}}
\def\bfi{{\mathbf i}}
\def\bfj{{\mathbf j}}
\def\bfk{{\mathbf k}}
\def\bfl{{\mathbf l}}
\def\bfm{{\mathbf m}}
\def\bfn{{\mathbf n}}
\def\bfo{{\mathbf o}}
\def\bfp{{\mathbf p}}
\def\bfq{{\mathbf q}}
\def\bfr{{\mathbf r}}
\def\bfs{{\mathbf s}}
\def\bft{{\mathbf t}}
\def\bfu{{\mathbf u}}
\def\bfv{{\mathbf v}}
\def\bfw{{\mathbf w}}
\def\bfx{{\mathbf x}}
\def\bfy{{\mathbf y}}
\def\bfz{{\mathbf z}}
%bold caps
\def\bfA{{\mathbf A}}
\def\bfB{{\mathbf B}}
\def\bfC{{\mathbf C}}
\def\bfD{{\mathbf D}}
\def\bfE{{\mathbf E}}
\def\bfF{{\mathbf F}}
\def\bfG{{\mathbf G}}
\def\bfH{{\mathbf H}}
\def\bfI{{\mathbf I}}
\def\bfJ{{\mathbf J}}
\def\bfK{{\mathbf K}}
\def\bfL{{\mathbf L}}
\def\bfM{{\mathbf M}}
\def\bfN{{\mathbf N}}
\def\bfO{{\mathbf O}}
\def\bfP{{\mathbf P}}
\def\bfQ{{\mathbf Q}}
\def\bfR{{\mathbf R}}
\def\bfS{{\mathbf S}}
\def\bfT{{\mathbf T}}
\def\bfU{{\mathbf U}}
\def\bfV{{\mathbf V}}
\def\bfW{{\mathbf W}}
\def\bfX{{\mathbf X}}
\def\bfY{{\mathbf Y}}
\def\bfZ{{\mathbf Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%bold symbols

\def\alphabf{\hbox{\boldmath$\alpha$\unboldmath}}
\def\betabf{\hbox{\boldmath$\beta$\unboldmath}}
\def\gammabf{\hbox{\boldmath$\gamma$\unboldmath}}
\def\deltabf{\hbox{\boldmath$\delta$\unboldmath}}
\def\epsilonbf{\hbox{\boldmath$\epsilon$\unboldmath}}
\def\zetabf{\hbox{\boldmath$\zeta$\unboldmath}}
\def\etabf{\hbox{\boldmath$\eta$\unboldmath}}
\def\iotabf{\hbox{\boldmath$\iota$\unboldmath}}
\def\kappabf{\hbox{\boldmath$\kappa$\unboldmath}}
\def\lambdabf{\hbox{\boldmath$\lambda$\unboldmath}}
\def\mubf{\hbox{\boldmath$\mu$\unboldmath}}
\def\nubf{\hbox{\boldmath$\nu$\unboldmath}}
\def\xibf{\hbox{\boldmath$\xi$\unboldmath}}
\def\pibf{\hbox{\boldmath$\pi$\unboldmath}}
\def\rhobf{\hbox{\boldmath$\rho$\unboldmath}}
\def\sigmabf{\hbox{\boldmath$\sigma$\unboldmath}}
\def\taubf{\hbox{\boldmath$\tau$\unboldmath}}
\def\upsilonbf{\hbox{\boldmath$\upsilon$\unboldmath}}
\def\phibf{\hbox{\boldmath$\phi$\unboldmath}}
\def\chibf{\hbox{\boldmath$\chi$\unboldmath}}
\def\psibf{\hbox{\boldmath$\psi$\unboldmath}}
\def\omegabf{\hbox{\boldmath$\omega$\unboldmath}}
\def\inftybf{\hbox{\boldmath$\infty$\unboldmath}}
\def\hSigmabf{\hbox{$\widehat{\bf \Sigma}$}}
\def\Sigmabf{\hbox{$\bf \Sigma$}}
\def\Upsilonbf{\hbox{$\bf \Upsilon$}}
%\def\Phibf{\hbox{$\bf \Phi$}}
%\def\Psibf{\hbox{$\bf \Psi$}}
\def\Omegabf{\hbox{$\bf \Omega$}}
\def\Deltabf{\hbox{$\bf \Delta$}}
\def\Gammabf{\hbox{$\bf \Gamma$}}
\def\Thetabf{\hbox{$\bf \Theta$}}
\def\Lambdabf{\mbox{$ \bf \Lambda $}}
\def\Xibf{\hbox{\bf$\Xi$}}
\def\Pibf{{\bf \Pi}}
%\def\thetabf{\hbox{\boldmath$\theta$\unboldmath}}
\def\thetabf{{\mbox{\boldmath$\theta$\unboldmath}}}
%\def\thetabf{\hbox{$\bf{\theta}$}}
\def\Upsilonbf{\hbox{\boldmath$\Upsilon$\unboldmath}}
\newcommand{\Phibf}{\mbox{${\bf \Phi}$}}
\newcommand{\Psibf}{\mbox{${\bf \Psi}$}}
\def\olambda{\mathfrak{o}(\lambda)}
\def\complex{\mathfrak{C}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Calligraphic
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
%\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%mathbb
\def\Abb{{\mathbb A}}
\def\BBb{{\mathbb B}}% different
\def\Cbb{{\mathbb C}}
\def\Dbb{{\mathbb D}}
\def\Ebb{{\mathbb E}}
\def\Fbb{{\mathbb F}}
\def\Gbb{{\mathbb G}}
\def\Hbb{{\mathbb H}}
\def\Ibb{{\mathbb I}}
\def\Jbb{{\mathbb J}}
\def\Kbb{{\mathbb K}}
\def\Lbb{{\mathbb L}}
\def\Mbb{{\mathbb M}}
\def\Nbb{{\mathbb N}}
\def\Obb{{\mathbb O}}
\def\Pbb{{\mathbb P}}
\def\Qbb{{\mathbb Q}}
\def\Rbb{{\mathbb R}}
\def\Sbb{{\mathbb S}}
\def\Tbb{{\mathbb T}}
\def\Ubb{{\mathbb U}}
\def\Vbb{{\mathbb V}}
\def\Wbb{{\mathbb W}}
\def\Xbb{{\mathbb X}}
\def\Ybb{{\mathbb Y}}
\def\Zbb{{\mathbb Z}}

\def\hbfP{{\widehat{\bfP}}}

\def\tilf{{\widetilde{f}}}

\def\tilo{{\widetilde{o}}}
\def\tilomega{{\widetilde{\omega}}}

\def\tilJbf{{\widetilde{\bfJ}}}

%\def\tilJ{{\widetilde{J}}}
\def\tilO{{\widetilde{O}}}
%\def\tilP{{\widetilde{P}}}
\def\tilR{{\widetilde{R}}}

\def\tilAbf{{\widetilde{\bfA}}}
\def\tilJbf{{\widetilde{\bfJ}}}
\def\tilRbf{{\widetilde{\bfR}}}


\def\tilEbb{{\widetilde{\Ebb}}}
\def\tilPbb{{\widetilde{\Pbb}}}


\def\tiltilEbb{{\widetilde{\widetilde{\Ebb}}}}
\def\tiltilP{{\widetilde{\widetilde{P}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%command abbreviations
\newcommand{\bprfof}{\begin{proof_of}}
\newcommand{\eprfof}{\end{proof_of}}
\newcommand{\bprf}{\begin{myproof}}
\newcommand{\eprf}{\end{myproof}}
\newcommand{\bp}{\begin{psfrags}}
\newcommand{\ep}{\end{psfrags}}
\newcommand{\bl}{\begin{lemma}}
\newcommand{\el}{\end{lemma}}
\newcommand{\bt}{\begin{theorem}}
\newcommand{\et}{\end{theorem}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bd}{\begin{definition}}
\newcommand{\ed}{\end{definition}}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}\noindent}
\def\beqn{\begin{eqnarray}}
\def\eeqn{\end{eqnarray} \noindent}
\def\beqnn{  \begin{eqnarray*}}
\def\eeqnn{\end{eqnarray*}  \noindent}
\def\bcase{  \begin{numcases}}
\def\ecase{\end{numcases}   \noindent}
\def\bsbcase{  \begin{subnumcases}}
\def\esbcase{\end{subnumcases}   \noindent}

\def\endproof{\hfill$\blacksquare$}
\def\defeq{{:=}}%{{\stackrel{\Delta}{=}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%theorems

\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{problem}{Problem}
\newtheorem{assumption}{A}
\newtheorem{properties}{Properties}
\newtheorem{conjecture}{Conjecture}
\newtheorem{criterion}{Criterion}
\newtheorem{proposition}{Proposition}
\newtheorem{notation}{Notation}
\newtheorem{derivation}{Derivation}
\newtheorem{claim}{Claim}
\newtheorem{observation}{Observation}
\newtheorem{fact}{Fact}

%\theoremstyle{definition}
\newtheorem{definition}{Definition}
%\theorembodyfont{\upshape} %body not italicized

%\theoremstyle{remark} %Comment it if you want to make the style of remarks the same as theorems
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
%\theoremheaderfont{\normalfont\bfseries}
%\theorembodyfont{\normalfont}
%\newtheorem{example}{Example}
%\newtheorem{proof}{Proof}

\newenvironment{myproof}{\noindent{\bf Proof:} \hspace*{1em}}{
    \hspace*{\fill} $\Box$ }
\newenvironment{proof_of}[1]{\noindent {\bf Proof of #1: }}{\hspace*{\fill} $\Box$ }
\newenvironment{proof_claim}{\begin{quotation} \noindent}{
    \hspace*{\fill} $\diamond$ \end{quotation}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\matplottc}[1]{               % single matlab plot twocolumn
        \unitlength .45truein
        \begin{center}
%         \begin{picture}(5,4.6)(1.05,.45)
        \special{psfile=#1.ps hscale=50 vscale=50}
        \end{picture}
        \end{center}
}
\newcommand{\matplotfp}[1]{               % single matlab plot fullpage
        \unitlength .45truein
        \begin{center}
        \begin{picture}(14,16)(.8,-1)
        \special{psfile=#1.ps hscale=100 vscale=100}
        \end{picture}
        \end{center}
}
\newcommand{\matplothp}[1]{               % single matlab plot halfpage
        \unitlength .45truein
        \begin{center}  \begin{picture}(14,7.5)(-1,.55)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplothptop}[1]{               % single matlab plot halfpage
        \unitlength .45truein                % when figure is top of page
        \begin{center}  \begin{picture}(14,6.3)(-1,1.15)
        \special{psfile=#1.ps hscale=80 vscale=80}
        \end{picture}
        \end{center}
}
\newcommand{\matplotcc}[4]{             % two axis('square') plots side by side
        \vspace{2.8in}
        \special{psfile=#1.ps voffset=-10 hoffset=-22 vscale=52 hscale=52}
        \special{psfile=/user/xu/isl/matlab/psfiles/#2.ps voffset=-10 hoffset=213 vscale=52 hscale=52}
        \hspace*{\fill}\hspace*{0.35in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.35in}#4\hspace*{\fill} }
\newcommand{\matplottwo}[4]{             % two axis('normal') plots side by side
        \vspace{2.62in}
        \special{psfile=#1.ps voffset=-10 hoffset=-27 vscale=52 hscale=52}
        \special{psfile=#2.ps voffset=-10 hoffset=218 vscale=52 hscale=52}
        \vspace*{0.18in}
        \hspace*{\fill}\hspace*{-.05in}#3\hspace*{\fill}\hspace*{\fill}\hspace*{
0.65in}#4\hspace*{\fill} } %%
%% This is for making fancy paragraphs
%%
\def\psfancypar#1#2{\begingroup\def\par{\endgraf\endgroup\lineskiplimit=0pt}
               \setbox2=\hbox{\large\sc #2}
%              \showthe\lht2\showthe\baselineskip
               \newdimen\tmpht \tmpht \ht2 \advance\tmpht by \baselineskip
%              \showthe\tmpht
% Changed 10/2/89 rhr - t-bol -> Times-Bold for dvi2ps to dvips conversion
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
%              \showthe\ht1
               \count7=\tmpht \count8=\ht1
%  note that all this BS is necessary since TeX only does integer
%  divides and rounds all results
               \divide\count8 by 1000 \divide\count7 by \count8
%               \showthe\count7
               \tmpht=.001\tmpht\multiply\tmpht by \count7
%               \showthe\tmpht
%              \font\hhuge=t-bol at \tmpht
               \font\hhuge=Times-Bold at \tmpht
               \setbox1=\hbox{{\hhuge #1}}
               \noindent
                \hangindent1.05\wd1
               \hangafter=-2 {\hskip-\hangindent
               \lower1\ht1\hbox{\raise1.0\ht2\copy1}%
                \kern-0\wd1}\copy2\lineskiplimit=-1000pt}


\newenvironment{ap}{
\renewcommand{\thesection}{\mbox{Appendix }\Alph{section}}
\renewcommand{\thesubsection}{\Alph{section}.\arabic{subsection
}}
\renewcommand{\theequation}{\mbox{\Alph{section}.}\arabic{equation}}
}{
\renewcommand{\thesection}{\arabic{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\renewcommand{\theequation}{\arabic{equation}}
}



\def\Kout{\setbox1=\hbox{\Huge\bf K}\hbox to
1.05\wd1{\hspace{.05\wd1}\special{
"/Times-BoldItalic findfont 25 scalefont setfont
/prKzip
{0 0 moveto (K) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prKzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prKzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (K) true charpath  stroke
 grestore
} def
dozip}}}
\def\Sout{\setbox1=\hbox{\Huge\bf S}\hbox to 1.05\wd1{\hspace{.05\wd1}\special{"
/Times-BoldItalic findfont 25 scalefont setfont
/prSzip
{0 0 moveto (S) show} def
/dozip
{gsave
  /xp 0 def
  .08 -.04 0
  {
   setgray
  prSzip
%  /xp xp dx add def xp -.7 translate %for
  -.7 .4 translate} for
  1 setgray prSzip
  0 0 moveto
  0 setgray
  .5 setlinewidth
  (S) true charpath  stroke
 grestore
} def
dozip}}}
\newcommand{\hKbf}{\mbox{${\widehat{\bfK}}$}}
\newcommand{\hthetabf}{\mbox{${\widehat{\thetabf}}$}}
\newcommand{\hmubf}{\mbox{${\widehat{\mubf}}$}}
%\newcommand{\thbar}{\mbox{${\bar{\thetabf}}_N$}}
%\newcommand{\etahat}{\mbox{${\hat{\etabf}}$}}
%\newcommand{\etabf}{\mbox{${\bf\eta}$}}
%\newcommand{\e}{\mbox{${\bf e}_k$}}
%\newcommand{\ehat}{\mbox{$\hat{\bf e}_k$}}
%\newcommand{\EWE}{\mbox{${\bf E}_s^{}{\bf WE}_s^*$}}
%\newcommand{\DPD}{\mbox{$\Dbf^*\Pbf_{\bf A}^{\perp} \Dbf$}}
%\newcommand{\EWEhat}{\mbox{$\hat{\bf E}_s^{}{\bf W}\hat{\bf E}_s^*$}}
%\newcommand{\E}{\mbox{{\rm E}}}
%\newcommand{\Efs}{\mbox{${\bf E}_s^{}$}}
%\newcommand{\En}{\mbox{${\bf E}_n^{}$}}
%\newcommand{\Eshat}{\mbox{$\hat{\bf E}_s^{}$}}
%\newcommand{\Lshat}{\mbox{$\hat {\bf \Lambda}_s^{}$}}
%\newcommand{\Ls}{\mbox{$ {\bf \Lambda}_s^{}$}}
%\newcommand{\Ln}{\mbox{$ {\bf \Lambda}_n^{}$}}
%\newcommand{\Ltilde}{\mbox{$\widetilde {\bf \Lambda}$}}
%\newcommand{\Enhat}{\mbox{$\hat{\bf E}_n^{}$}}
%\newcommand{\Lnhat}{\mbox{$\hat {\bf \Lambda}_n^{}$}}
%\newcommand{\Ai}{\mbox{$ ({\bf A}^*{\bf A})^{-1} $}}
%\newcommand{\abf}{\mbox{${\bf a}$}}


%Define affiliation at footnote
% Make \small be smaller (8 pt)
%\def\small{\@setsize\small{9pt}\viiipt\@viiipt\let\@listi\@listI}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Macros to restate theorems in appendices
%
% Use as follows:
%\torestate{Theorem}{thm:restate}{If $x \in \N$ then $x+1 \in \N$.}
%
%\restate{thm:restate}

\newcommand{\torestate}[3]{%
\expandafter \def \csname BBRESTATE #2 \endcsname{#3}
\theoremstyle{plain}
\newtheorem{BBRESTATETHMNUM#2}[theorem]{#1}
\begin{BBRESTATETHMNUM#2}\label{#2}\csname BBRESTATE #2 \endcsname   \end{BBRESTATETHMNUM#2}
\newtheorem*{BBRESTATETHMNONNUM#2}{{#1}~\ref{#2}}
}


\newcommand{\restate}[1]{\begin{BBRESTATETHMNONNUM#1}[Restated] \csname BBRESTATE #1 \endcsname
\end{BBRESTATETHMNONNUM#1}}


\definecolor{blue1}{HTML}{0066FF}
\definecolor{lpurple}{cmyk}{.05,0.18,0,0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



